Blockchain in Supply Chain: Opportunities and Design Considerations

Supply chain applications operate in a multi-stakeholder setting, demanding trust, provenance, and transparency. Blockchain technology provides mechanisms to establish a decentralized infrastructure involving multiple stakeholders. Such mechanisms make the blockchain technology ideal for multi-stakeholder supply chain applications. This chapter introduces the characteristics and requirements of the supply chain and explains how blockchain technology can meet the demands of supply chain applications. In particular, this chapter discusses how data and trust management can be established using blockchain technology. The importance of scalability and interoperability in a blockchain-based supply chain is highlighted to help the stakeholders make an informed decision. The chapter concludes by underscoring the design challenges and open opportunities in the blockchain-based supply chain domain.

==> table.tex <==
\begin{table}[]
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Source}}                                     & \multicolumn{1}{c|}{\textbf{Definition and Solution}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|c|}{Sensing Latency}                                     & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} Sensing is fundamental to IoT applications, wherein not all the \\ sensors behave in the same way. For phenomena that move through space \\ slowly (such as acoustic vibrations or moving objects), it may not be easy \\ to sense the data in real-time.\\ \textbf{Potential Solution:} One solution to improve this would be to place sensors \\ more densely so they can detect the object or the phenomenon of interest quickly.\end{tabular}                                                                            \\ \hline
\multicolumn{1}{|c|}{Propagation Latency}                                 & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} How far does data have to travel to be processed? In some cases, \\ the nearest cloud infrastructure could be in a different city or a country. \\ \textbf{Potential Solution:} Rely on a cloud infrastructure that is close to the \\ application environment. Edge or Fog computing can solve this problem.\end{tabular}                                                                                                                                                                                             \\ \hline
Transmission Latency                                                       & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} The time it takes for a packet to travel from one device to \\ another device through a wired or wireless link. For a single packet this \\ depends on the link rate.\\ \textbf{Potential Solution:} Higher data rates can be helpful to reduce transmission \\ latency.\end{tabular}                                                                                                                                                                                                                                  \\ \hline
Retransmission Latency                                                    & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} The time it takes for a packet to reach the desired destination \\ after retransmissions. Note that the retransmissions happen due to \\ poor link performance.\\ \textbf{Potential Solution:} Having more reliable links means fewer \\ retransmissions to send packets successfully, which would result in lower \\ link delay; this may be enabled by increasing radio power or by utilizing \\ forward error correction, which may incur higher hardware complexity in \\ some cases.\end{tabular} \\ \hline
Scheduling Latency                                                        & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} In time-synchronized networks such as TSCH, nodes have to \\ wait for their turn to transmit or receive data. Such waiting times introduce \\ scheduling latency.\\ \textbf{Potential Solution:} Optimized designs may be needed or alternative schemes \\ that allow limited random access in case of time-critical data may be helpful \\ in some cases.\end{tabular}                                                                                                                                                \\ \hline
Encounter Latency                                                         & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} For intermittently connected mobile networks (ICMN), such \\ as when mobile devices are used as data mules, carriers for data from \\ static sensors, a source of latency could be how long you have to wait \\ for a mobile carrier to show up.\\ \textbf{Potential Solution:} It is difficult to provide real-time guarantees in mobile \\ scenarios. Application developers should account for the transient connectivity \\ at the design phase.\end{tabular}                                                      \\ \hline
Delivery Latency                                                          & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} In ICMN networks, the delivery latency depends on the \\ routing scheme.\\ \textbf{Potential Solution:} Flooding or multi-copy routing is the fastest \\ delivery mechanism for low data rate applications; but single-copy \\ routing is more energy efficient.\end{tabular}                                                                                                                                                                                                                                          \\ \hline
Queuing Latency                                                           & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} Network congestion may lead to queuing latency.\\ \textbf{Potential Solution:} Congestion control mechanisms, as well as \\ scheduling mechanisms that avoid congestion, can reduce queuing latency.\end{tabular}                                                                                                                                                                                                                                                                                                       \\ \hline
\begin{tabular}[c]{@{}l@{}}Processing Hardware \\ Latency\end{tabular}    & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} The time it takes for a CPU or GPU to process the data.\\ \textbf{Potential Solution:} Faster device/edge processors and multi-processor \\ scheduling techniques can reduce processing latency.\end{tabular}                                                                                                                                                                                                                                                                                                                     \\ \hline
\begin{tabular}[c]{@{}l@{}}Processing Algorithmic \\ Latency\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Definition:} The time it takes for an algorithm to compute the result.\\ \textbf{Potential Solution:} Using lightweight algorithms or machine learning models \\ that can compute quickly even with limited resources can reduce the algorithmic latency.\end{tabular}                                                                                                                                                                                                                                                                               \\ \hline
\end{tabular}
\caption{Many Sources of Latency in IoT Systems.}
\label{tab:tab1}
\end{table}
